Provably Feedback-Efficient Reinforcement Learning via Active Reward Learning

An appropriate reward function is of paramount importance in specifying a task in reinforcement learning (RL). Yet, it is known to be extremely challenging in practice to design a correct reward function for even simple tasks. Human-in-the-loop (HiL) RL allows humans to communicate complex goals to the RL agent by providing various types of feedback. However, despite achieving great empirical successes, HiL RL usually requires too much feedback from a human teacher and also suffers from insufficient theoretical understanding. In this paper, we focus on addressing this issue from a theoretical perspective, aiming to provide provably feedback-efficient algorithmic frameworks that take human-in-the-loop to specify rewards of given tasks. We provide an active-learning-based RL algorithm that first explores the environment without specifying a reward function and then asks a human teacher for only a few queries about the rewards of a task at some state-action pairs. After that, the algorithm guarantees to provide a nearly optimal policy for the task with high probability. We show that, even with the presence of random noise in the feedback, the algorithm only takes $\widetilde{O}(H{{\dim_{R}^2}})$ queries on the reward function to provide an $\epsilon$-optimal policy for any $\epsilon > 0$. Here $H$ is the horizon of the RL environment, and $\dim_{R}$ specifies the complexity of the function class representing the reward function. In contrast, standard RL algorithms require to query the reward function for at least $\Omega(\operatorname{poly}(d, 1/\epsilon))$ state-action pairs where $d$ depends on the complexity of the environmental transition.

==> related.tex <==

{\color{red}
Our active reward learning algorithm is inspired by a line of works~\citep{cesa2009robust,dekel2010robust,agarwal2013selective} considering online classification problems. Our reward-free exploration algorithm is most relevant to \citet{wu2021accommodating,wang2020reward} studying reward-free RL in tabular/linear setting. Due to space limit, more related works are deferred to Appendix~\ref{related1}.}


==> tech.tex <==
\begin{lem}[\citep{freedman1975tail}]
\label{lem:freedman}
Consider a real-valued martingale $\{Y_k:k=0,1,2...\}$ with difference sequence $\{X_k:k=1,2,...\}$. Assume that the difference sequence is uniformly bounded:
\[
|X_k|\leq R \text{ almost surely for } k=1,2,3,...  \text{.}
\]
For a fixed $n\in\mathbb{N}$, assume that
$$
\sum_{k=1}^n\mathbb{E}_{k-1}(X_k^2)\leq\sigma^2 $$
almost surely.
Then for all $t\geq 0$,
\[
P\{|Y_n-Y_0|\geq t\}\leq 2\exp\left\lbrace -\frac{t^2/2}{\sigma^2+Rt/3}\right\rbrace.
\]
\end{lem}
\begin{lem}[Vector version of Hoeffding's inequality]
\label{lem:vechoeffding}
Let $A\in\RR^{m\times n}$ be a matrix. Let $\xi_1,\xi_2,...,\xi_n$ be independent, mean-zero and $\sigma$-subgaussian random variables. Then for any $\delta>0$,
\[
P\left(\|A\xi\|_2^2\geq 2\sigma^2 \log\frac{2m}{\delta}\trace(AA^T)\right)\leq \delta
\]
where $\xi=(\xi_1,\xi_2,...,\xi_n)^T$.
\end{lem}
\begin{lem}[Elliptical potential lemma]
Let $V_0$ be a positive definite matrix in $\RR^{d\times d}$. Let $a_1,...,a_n$ be a sequence of vectors in $\RR^d$ with $\|a_t\|_2\leq L<\infty$. For all $t\in[n]$, let $V_t=V_0+\sum_{s\leq t}a_s a_s^T$. Then,
\[
\sum_{t=1}^n \left(1\land \|a_t\|^2_{V_{t-1}^{-1}}\right)\leq 2\log\left(\frac{\det V_n}{\det V_0}\right)\leq 2d\log\left(\frac{\trace V_0+nL^2}{d\det(V_0)^{1/d}}\right)
\].
\end{lem}
